Patterns of gender-specializing query reformulation

Users of search systems often reformulate their queries by adding query terms to reflect their evolving information need or to more precisely express their information need when the system fails to surface relevant content. Analyzing these query reformulations can inform us about both system and user behavior. In this work, we study a special category of query reformulations that involve specifying demographic group attributes, such as gender, as part of the reformulated query (e.g., "olympic 2021 soccer results" to "olympic 2021 women's soccer results"). There are many ways a query, the search results, and a demographic attribute such as gender may relate, leading us to hypothesize different causes for these reformulation patterns, such as under-representation on the original result page or based on the linguistic theory of markedness. This paper reports on an observational study of gender-specializing query reformulations -- their contexts and effects -- as a lens on the relationship between system results and gender, based on large-scale search log data from Bing. We find that these reformulations sometimes correct for and other times reinforce gender representation on the original result page, but typically yield better access to the ultimately-selected results. The prevalence of these reformulations -- and which gender they skew towards -- differ by topical context. However, we do not find evidence that either group under-representation or markedness alone adequately explains these reformulations. We hope that future research will use such reformulations as a probe for deeper investigation into gender (and other demographic) representation on the search result page.

==> 04-identify.tex <==
%\section{Identifying query reformulations for group-based specialization}
\section{Identifying query reformulations for gender-based specialization}
\label{sec:identify}
Our study focuses on query reformulation patterns that specializes the information need to specific gender groups.
We adopt a slightly stricter definition of specializing query reformulations compared to Liu et al.~\citep{liu2010analysis, liu2010analysis2}.
We define a query reformulation to be specializing if the reformulated query contains all the terms in-order as in the original query and includes an additional set of contiguous terms added anywhere to the original query.
Finally, to define group-based specialization we enforce an additional constraint that the additional set of contiguous terms can only belong either to a list of known terms describing demographic group attributes---\eg, for gender we consider ``woman'', ``man'', ``women'', ``men'', ``woman's'', ``man's'', ``women's'', ``men's'', ``womans'', ``mans'', ``womens'', ``mens'', ``female'', ``male'', ``male's'', ``female's'', ``males'', and ``females''---or a list of prepositions---\eg, ``about'', ``against'', ``according to'', ``among'', ``at'', ``by'', ``except'', ``for'', ``from'', ``in'', ``like'', ``of'', ``on'', ``to'', ``with'', and ``without''.
In line with this definition, we would consider the reformulations ``olympic 2021 soccer results'' $\to$ ``olympic 2021 \emph{women's} soccer results'' and ``bmi calculator'' $\to$ ``bmi calculator \emph{for men}'' as query reformulations performing group-based specializations.
Given large-scale search logs we can automatically identify instances of query reformulations matching these specified patterns. 

\ifincludeappendix
To consider other demographic groups beyond gender, it would be convenient if we can (semi-)automatically detect other relevant group terms. Please see Appendix~\ref{sec:appendix-extend} for more details.
\fi

%\todo{Describe a general method for identifying query reformulations that explicitly add demographic attributes.}

%In our work, we want to analyze queries that were reformulated for demographic attributes. To do that, first we need to identify the common demographic attributes that user use to reformulate the queries. In this section, we will introduce a strategy to find common demographic groups and the queries that get reformulated for those groups.

%\begin{itemize}
%    \item At first, we used a seed demographic attribute- gender to find queries that are commonly reformulated for that groups. We used binary gender and the representative terms associated with it for example, "men", "women", "male", "female" etc.
%    \item We extracted query-reformulation pair where the reformulation occurred for any binary gender terms. For example, the query "soccer" is reformulated as "soccer for women". 
%    \item After extracting a set of binary gender-based reformulated queries, we used those queries to further identify other group information. Since, these queries are already reformulated for a demographic attribute, we believe that analysing other reformulation of these queries will elicit different group information that users commonly use to reformulate. We extract the all the reformulation for the binary gender-based queries that we got from step 2 using the template- "original query + for + <place holder>".
%    \item The derived data came with noise- terms that are not representative of any demographic groups. As a filtering step, we manually identified the demographic groups attributes, for example, "teens", "kids", "black men" etc.
%    \item We observed that there are both independent and inter-sectional group attributes, ...
%    \item We categorized the terms in various groups attributes like, age, race and repeat step 1 to find query-reformulation pair for a group.
%\end{itemize}

